Contrastive Enhanced Slide Filter Mixer for Sequential Recommendation

Sequential recommendation (SR) aims to model user preferences by capturing behavior patterns from their item historical interaction data. Most existing methods model user preference in the time domain, omitting the fact that users' behaviors are also influenced by various frequency patterns that are difficult to separate in the entangled chronological items. However, few attempts have been made to train SR in the frequency domain, and it is still unclear how to use the frequency components to learn an appropriate representation for the user. To solve this problem, we shift the viewpoint to the frequency domain and propose a novel Contrastive Enhanced \textbf{SLI}de Filter \textbf{M}ixEr for Sequential \textbf{Rec}ommendation, named \textbf{SLIME4Rec}. Specifically, we design a frequency ramp structure to allow the learnable filter slide on the frequency spectrums across different layers to capture different frequency patterns. Moreover, a Dynamic Frequency Selection (DFS) and a Static Frequency Split (SFS) module are proposed to replace the self-attention module for effectively extracting frequency information in two ways. DFS is used to select helpful frequency components dynamically, and SFS is combined with the dynamic frequency selection module to provide a more fine-grained frequency division. Finally, contrastive learning is utilized to improve the quality of user embedding learned from the frequency domain. Extensive experiments conducted on five widely used benchmark datasets demonstrate our proposed model performs significantly better than the state-of-the-art approaches. Our code is available at https://github.com/sudaada/SLIME4Rec.

==> experiments.tex <==
Table II presents the recommendation performance of all methods on the six datasets(\textbf{RQ1}). By considering the second 

\pgfplotsset{
axis background/.style={fill=gallery},
grid=both,
  xtick pos=left,
  ytick pos=left,
  tick style={
    major grid style={style=white,line width=1pt},
    minor grid style=bgc,
    draw=none
    },
  minor tick num=1,
  ymajorgrids,
	major grid style={draw=white},
	y axis line style={opacity=0},
	tickwidth=0pt,
}


\begin{figure*}[]
\centering
    \begin{tikzpicture}[scale=0.5]
	\begin{groupplot}[
	    group style={group size=4 by 1,
	        horizontal sep = 42pt}, 
	    width=0.5\textwidth,
	    height=0.4\textwidth,
	   % xlabel=\large layers,
        ylabel=NDCG@10,
        % xticklabels={16, 32, 64, 128, 256},
        % xtick={1,2,3,4,5},
        ymajorgrids,
        major grid style={draw=white},
        y axis line style={opacity=0},
        tickwidth=0pt,
        yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
        },
        scaled y ticks=false,
        every axis title/.append style={at={(0.1,0.8)},font=\bfseries}
	    ]
		\nextgroupplot[
		legend style = {
		  font=\small,
          draw=none, 
          fill=none,
          column sep = 1pt, 
          /tikz/every even column/.append style={column sep=5mm},
          legend columns = -1, 
          legend to name = grouplegend},
        xlabel=\large L,
        xticklabels={1,2,3,4,5,6,7,8},
        xtick={1,2,3,4,5,6,7,8},
		]
		
		\addplot[thick,color=tuatara,mark=pentagon] coordinates {
          (1, 0.0594)
          (2, 0.062)
          (3, 0.0563)
          (4, 0.0527)
          (5, 0.0508)
          (6, 0.0429)
          (7, 0.0421)
          (8, 0.0408)
        }; \addlegendentry{DM4Rec}
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (1, 0.0476)
          (2, 0.0499)
          (3, 0.0499)
          (4, 0.0528)
          (5, 0.0472)
          (6, 0.0503)
          (7, 0.0518)
          (8, 0.0524)
        }; \addlegendentry{SASRec}
        \addplot[thick,color=matisse,mark=square] coordinates {
          (1, 0.0312)
          (2, 0.0316)
          (3, 0.0321)
          (4, 0.0249)
          (5, 0.0338)
          (6, 0.0339)
          (7, 0.0302)
          (8, 0.0314)
        };\addlegendentry{BERT4Rec}
        \addplot[thick,color=sun_shade,mark=diamond] coordinates {
          (1, 0.0386)
          (2, 0.0432)
          (3, 0.0399)
          (4, 0.0381)
          (5, 0.043)
          (6, 0.0391)
          (7, 0.0409)
          (8, 0.0405)
        };\addlegendentry{GRU4Rec}
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (1, 0.0356)
          (2, 0.0356)
          (3, 0.0356)
          (4, 0.0356)
          (5, 0.0356)
          (6, 0.0356)
          (7, 0.0356)
          (8, 0.0356)
        };\addlegendentry{Caser}
        
        \nextgroupplot[
        xlabel=\large D,
        xticklabels={32, 64, 96, 128, 256},
        xtick={1,2,3,4,5},]
		\addplot[thick,color=tuatara,mark=pentagon] coordinates {
          (1, 0.0594)
          (2, 0.0505)
          (3, 0.0515)
          (4, 0.0495)
          (5, 0.0419)
        };
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (1, 0.0473)
          (2, 0.0486)
          (3, 0.0506)
          (4, 0.0467)
          (5, 0.0465)
        };
        \addplot[thick,color=matisse,mark=square] coordinates {
          (1, 0.0412)
          (2, 0.0326)
          (3, 0.0345)
          (4, 0.0334)
          (5, 0.0381)
        };
        \addplot[thick,color=sun_shade,mark=diamond] coordinates {
          (1, 0.0408)
          (2, 0.0395)
          (3, 0.0424)
          (4, 0.0397)
          (5, 0.0392)
        };
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (1, 0.0429)
          (2, 0.0374)
          (3, 0.0432)
          (4, 0.0391)
          (5, 0.0373)
        };
        
        \nextgroupplot[
        xlabel=\large n,
        xticklabels={25,50,100,150,200},
        xtick={1,2,3,4,5},
        ]
		\addplot[thick,color=tuatara,mark=pentagon] coordinates {
          (1, 0.0526)
          (2, 0.0594)
          (3, 0.0503)
          (4, 0.0538)
          (5, 0.0554)
        };
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (1, 0.0476)
          (2, 0.0501)
          (3, 0.0476)
          (4, 0.0484)
          (5, 0.0482)
        };
        \addplot[thick,color=matisse,mark=square] coordinates {
          (1, 0.0432)
          (2, 0.0386)
          (3, 0.0381)
          (4, 0.0394)
          (5, 0.0343)
        };
        \addplot[thick,color=sun_shade,mark=diamond] coordinates {
          (1, 0.0429)
          (2, 0.0369)
          (3, 0.0396)
          (4, 0.0405)
          (5, 0.0373)
        };
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (1, 0.0439)
          (2, 0.0385)
          (3, 0.0376)
          (4, 0.0417)
          (5, 0.0362)
        };
        
        \nextgroupplot[
        xlabel=\large p,
        xticklabels={0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9},
        xtick={1,2,3,4,5,6,7,8,9},
        ]
		\addplot[thick,color=tuatara,mark=pentagon] coordinates {
          (1, 0.0559)
          (2, 0.0541)
          (3, 0.056)
          (4, 0.0575)
          (5, 0.0556)
          (6, 0.0562)
          (7, 0.0563)
          (8, 0.0543)
          (9, 0.0594)
        };
         \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
          (1, 0.05)
          (2, 0.0492)
          (3, 0.0497)
          (4, 0.0476)
          (5, 0.0465)
          (6, 0.0468)
          (7, 0.0458)
          (8, 0.0512)
          (9, 0.0479)
        };
        \addplot[thick,color=matisse,mark=square] coordinates {
          (1, 0.0327)
          (2, 0.0346)
          (3, 0.0284)
          (4, 0.0313)
          (5, 0.0277)
          (6, 0.0338)
          (7, 0.0387)
          (8, 0.0359)
          (9, 0.0415)
        };
        \addplot[thick,color=sun_shade,mark=diamond] coordinates {
          (1, 0.0396)
          (2, 0.0376)
          (3, 0.0408)
          (4, 0.0399)
          (5, 0.0415)
          (6, 0.0389)
          (7, 0.0406)
          (8, 0.0445)
          (9, 0.0408)
        };
        \addplot[thick,color=flamingo,mark=*] coordinates {
          (1, 0.0346)
          (2, 0.0352)
          (3, 0.0317)
          (4, 0.0342)
          (5, 0.0338)
          (6, 0.0355)
          (7, 0.0391)
          (8, 0.0374)
          (9, 0.0412)
        };
        
        
%         \nextgroupplot[
%         title=Beauty,
%         ylabel=NDCG@10,
%         xlabel=\large layers,
%         xticklabels={1,2,3,4,5,6,7,8,9},
%         xtick={1,2,3,4,5,6,7,8,9},
%         ]
% 		\addplot[thick,color=tuatara,mark=pentagon] coordinates {
%           (1, 0.0212)
%           (2, 0.0208)
%           (3, 0.0207)
%           (4, 0.0202)
%           (5, 0.0214)
%           (6, 0.0209)
%           (7, 0.021)
%           (8, 0.0201)
%           (9, 0.0204)
%         };
%         %  \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
%         %   (1, 0.0515)
%         %   (2, 0.0574)
%         %   (3, 0.0557)
%         %   (4, 0.057)
%         %   (5, 0.0585)
%         %   (6, 0.0563)
%         %   (7, 0.0573)
%         %   (8, 0.0552)
%         %   (9, 0.0545)
%         % };
%         % \addplot[thick,color=matisse,mark=square] coordinates {
%         %   (1, 0.1898)
%         %   (2, 0.2203)
%         %   (3, 0.2441)
%         %   (4, 0.2580)
%         %   (5, 0.2590)
%         % };
%         % \addplot[thick,color=sun_shade,mark=diamond] coordinates {
%         %   (1, 0.2264)
%         %   (2, 0.2567)
%         %   (3, 0.2662)
%         %   (4, 0.2672)
%         %   (5, 0.2653)
%         % };
%         % \addplot[thick,color=flamingo,mark=*] coordinates {
%         %   (1, 0.2488)
%         %   (2, 0.2839)
%         %   (3, 0.3047)
%         %   (4, 0.3034)
%         %   (5, 0.3025)
%         % };
        
%         \nextgroupplot[
%         title=Steam,
%         ylabel=NDCG@10]
% 		\addplot[thick,color=tuatara,mark=pentagon] coordinates {
%           (1, 0.2395)
%           (2, 0.2778)
%           (3, 0.3235)
%           (4, 0.3291)
%           (5, 0.3313)
%         };
%         %  \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
%         %   (1, 0.2848)
%         %   (2, 0.3278)
%         %   (3, 0.3501)
%         %   (4, 0.3559)
%         %   (5, 0.3594)
%         % };
%         % \addplot[thick,color=matisse,mark=square] coordinates {
%         %   (1, 0.2482)
%         %   (2, 0.2696)
%         %   (3, 0.2834)
%         %   (4, 0.2870)
%         %   (5, 0.2857)
%         % };
%         % \addplot[thick,color=sun_shade,mark=diamond] coordinates {
%         %   (1, 0.2897)
%         %   (2, 0.3492)
%         %   (3, 0.3737)
%         %   (4, 0.3752)
%         %   (5, 0.3783)
%         % };
%         % \addplot[thick,color=flamingo,mark=*] coordinates {
%         %   (1, 0.3534)
%         %   (2, 0.3882)
%         %   (3, 0.4007)
%         %   (4, 0.4013)
%         %   (5, 0.3998)
%         % };
        
%         \nextgroupplot[
%         title=ML-1m,
%         ylabel=NDCG@10,
%         xlabel=\large layers,
%         xticklabels={1, 2, 4, 8, 16, 32, 64},
%         xtick={1,2,3,4,5,6,7},
%         ]
% 		\addplot[thick,color=tuatara,mark=pentagon] coordinates {
%           (1, 0.0208)
%           (2, 0.0217)
%           (3, 0.021)
%           (4, 0.0212)
%           (5, 0.0207)
%           (6, 0.0196)
%           (7, 0.0192)
%         };
%         %  \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
%         %   (1, 0.5233)
%         %   (2, 0.5684)
%         %   (3, 0.6184)
%         %   (4, 0.6281)
%         %   (5, 0.6351)
%         % };
%         % \addplot[thick,color=matisse,mark=square] coordinates {
%         %   (1, 0.5966)
%         %   (2, 0.6419)
%         %   (3, 0.6611)
%         %   (4, 0.6692)
%         %   (5, 0.6639)
%         % };
%         % \addplot[thick,color=sun_shade,mark=diamond] coordinates {
%         %   (1, 0.5556)
%         %   (2, 0.6493)
%         %   (3, 0.6720)
%         %   (4, 0.6677)
%         %   (5, 0.6629)
%         % };
%         % \addplot[thick,color=flamingo,mark=*] coordinates {
%         %   (1, 0.6060)
%         %   (2, 0.6609)
%         %   (3, 0.6955)
%         %   (4, 0.6997)
%         %   (5, 0.6970)
%         % };
        
%         \nextgroupplot[
%         title=ML-20m,
%         ylabel=NDCG@10,
%         xlabel=\large segment,
%         xticklabels={1, 2, 4, 8, 16, 32,64},
%         xtick={1,2,3,4,5,6,7},
%         ]
% 		\addplot[thick,color=tuatara,mark=pentagon] coordinates {
%           (1, 0.0213)
%           (2, 0.0203)
%           (3, 0.0199)
%           (4, 0.0199)
%           (5, 0.0203)
%           (6, 0.0201)
%           (7, 0.0203)
%         };
%         %  \addplot[thick,color=free_speech_aquamarine,mark=triangle*] coordinates {
%         %   (1, 0.5257)
%         %   (2, 0.6028)
%         %   (3, 0.6280)
%         %   (4, 0.6484)
%         %   (5, 0.6524)
%         % };
%         % \addplot[thick,color=matisse,mark=square] coordinates {
%         %   (1, 0.4415)
%         %   (2, 0.4922)
%         %   (3, 0.5295)
%         %   (4, 0.5399)
%         %   (5, 0.5427)
%         % };
%         % \addplot[thick,color=sun_shade,mark=diamond] coordinates {
%         %   (1, 0.4953)
%         %   (2, 0.5819)
%         %   (3, 0.6657)
%         %   (4, 0.6933)
%         %   (5, 0.7136)
%         % };
%         % \addplot[thick,color=flamingo,mark=*] coordinates {
%         %   (1, 0.5593)
%         %   (2, 0.6254)
%         %   (3, 0.6879)
%         %   (4, 0.7230)
%         %   (5, 0.7473)
%         % };
        
	\end{groupplot}
    \node at ($(group c1r1) + (370pt, 95pt)$) {\ref{grouplegend}};
    \end{tikzpicture}

    \caption{Performance comparision w.r.t. different $L,D,n,p$ on Music dataset.}
    \label{fig:dim_exp}
\end{figure*}


% 网络层数图
\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
    \centering
    \caption{Performance (HR@5) of the different filter module and the slide mode of frequency ramp structure. The best performance in each row is boldfaced.}
    \label{tab:seq}
    \begin{adjustbox}{max width=\linewidth}
            \begin{tabular}{cccccccccc}
            \toprule
            \multicolumn{2}{c}{\multirow{2}{*}{Method}}                               
            & \multicolumn{2}{c}{Beauty} 
            &
            & \multicolumn{2}{c}{Clothing}
            &
            & \multicolumn{2}{c}{Sportss}\\
            \cmidrule{3-4}
            \cmidrule{6-7}
            \cmidrule{9-10}
            \multicolumn{2}{c}{}
            & HR@5
            & NDCG@5
            &
            & HR@5
            & NDCG@5
            &
            & HR@5
            & NDCG@5\\
            
            \midrule
            \midrule
            \multirow{2}{*}{\textbf{2-Layer}} 
            & DuoRec
            & 0.0546
            & 0.0845
            &
            & 0.0193
            & 0.0302
            &
            & 0.0320
            & 0.0493\\
            
                         
            & \textbf{SLIME4Rec}
            & \textbf{0.0604}
            & \textbf{0.0903}
            &
            & \textbf{0.0225}
            & \textbf{0.0343}
            &
            & \textbf{0.0364}
            & \textbf{0.0561}\\
            
            %  下一行
            \midrule
            \multirow{2}{*}{\textbf{4-Layer}} 
            & DuoRec
            & 0.0551
            & 0.0855
            &
            & 0.0197
            & 0.0299
            &
            & 0.0315
            & 0.0480
            \\
            
            
            & \textbf{SLIME4Rec}
            & \textbf{0.0607}
            & \textbf{0.0920}
            &
            & \textbf{0.0221}
            & \textbf{0.0341}
            &
            & \textbf{0.0370}
            & \textbf{0.0572}
            \\
            
            %  下一行
            \midrule
            \multirow{2}{*}{\textbf{8-Layer}} 
            & DuoRec
            & 0.0565
            & 0.0867
            &
            & 0.0197
            & 0.0316
            &
            & 0.0299
            & 0.0460\\
            
            
            & \textbf{SLIME4Rec}
            & \textbf{0.0621}
            & \textbf{0.0910}
            &
            & \textbf{0.0221}
            & \textbf{0.0342}
            &
            & \textbf{0.0365}
            & \textbf{0.0563}\\
            
            %  下一行
            \midrule
            \multirow{2}{*}{\textbf{16-Layer}} 
            & DuoRec
            & 0.0517
            & 0.0790
            &
            & 0.0153
            & 0.0249\\
            
            
            & \textbf{SLIME4Rec}
            & \textbf{0.0585}
            & \textbf{0.0893}
            &
            & \textbf{0.0178}
            & \textbf{0.0274}\\
            
            % 底部
            \bottomrule
\end{tabular}   
    \end{adjustbox}
\end{table}

\begin{table}[t]
\renewcommand{\arraystretch}{1}
    \centering
    \label{tab:seq}
    \begin{adjustbox}{max width=\linewidth}
            \begin{tabular}{ccccccc}
            \toprule
            \multicolumn{2}{c}{\multirow{2}{*}{Method}}                               
            & \multicolumn{2}{c}{ML-1M} 
            &
            & \multicolumn{2}{c}{Yelp} \\
            \cmidrule{3-4}
            \cmidrule{6-7}
            \multicolumn{2}{c}{}
            & HR@5
            & NDCG@5
            &
            & HR@5
            & NDCG@5\\
            
            \midrule
            \midrule
            \multirow{2}{*}{\textbf{2-Layer}} 
            & DuoRec
            & 0.2038
            & 0.2946
            &
            & 0
            & 0\\
            
                         
            & \textbf{SLIME4Rec}
            & \textbf{0.2139}
            & \textbf{0.3026}
            &
            & \textbf{0}
            & \textbf{0}\\
            
            %  下一行
            \midrule
            \multirow{2}{*}{\textbf{4-Layer}} 
            & DuoRec
            & 0.2065
            & 0.2917
            &
            & 0
            & 0\\
            
            
            & \textbf{SLIME4Rec}
            & \textbf{0}
            & \textbf{0}
            &
            & \textbf{0}
            & \textbf{0}\\
    
            
            %  下一行
            \midrule
            \multirow{2}{*}{\textbf{8-Layer}} 
            & DuoRec
            & 0.2164
            & 0.3063
            &
            & 0
            & 0\\
            
            
            & \textbf{SLIME4Rec}
            & \textbf{0}
            & \textbf{0}
            &
            & \textbf{0}
            & \textbf{0}\\
            
            %  下一行
            \midrule
            \multirow{2}{*}{\textbf{16-Layer}} 
            & DuoRec
            & 0.0119
            & 0.0187
            &
            & 0
            & 0\\
            
            
            & \textbf{SLIME4Rec}
            & \textbf{0}
            & \textbf{0}
            &
            & \textbf{0}
            & \textbf{0}\\
        
            % 底部
            \bottomrule
\end{tabular}   
    \end{adjustbox}
\end{table}


% 网络层数表
% 网络层数图
\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
    \centering
    \caption{Performance comparison of SLIME4Rec with DuoRec at different layers. The best performance in each row is boldfaced.}
    \label{tab:seq}
    \begin{adjustbox}{max width=\linewidth}
            \begin{tabular}{cccccccccc}
            \toprule
            \multicolumn{2}{c}{
            \multirow{2}{*}{Method}
            }
            &
            \multicolumn{2}{c}{Beauty} 
            &
            & 
            \multicolumn{2}{c}{Clothing}
            &
            & 
            \multicolumn{2}{c}{Sports}\\
            \cmidrule{3-4}
            \cmidrule{6-7}
            \cmidrule{9-10}
            \multicolumn{2}{c}{}
            & HR@5
            & NDCG@5
            &
            & HR@5
            & NDCG@5
            &
            & HR@5
            & NDCG@5\\
            
            \midrule
            \midrule
            \multirow{3}{*}{\textbf{2-Layer}} 
            & DuoRec
            & 0.0546
            & 0.0845
            &
            & 0.0193
            & 0.0302
            &
            & 0.0320
            & 0.0493\\
            
            
            
                         
            & \multirow{2}{*}{\textbf{SLIME4Rec}}
            & \textbf{0.0604}
            & \textbf{0.0903}
            &
            & \textbf{0.0225}
            & \textbf{0.0343}
            &
            & \textbf{0.0364}
            & \textbf{0.0561}\\
            
                         
            &
            & $\uparrow$10.62\%
            & $\uparrow$6.86\%
            &
            & $\uparrow$16.58\% 
            & $\uparrow$13.58\%
            &
            & $\uparrow$13.75\%
            & $\uparrow$13.79\%\\
            
            %  下一行
            \midrule
            \multirow{3}{*}{\textbf{4-Layer}} 
            & DuoRec
            & 0.0551
            & 0.0855
            &
            & 0.0197
            & 0.0299
            &
            & 0.0315
            & 0.0480
            \\
            
            
            & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{SLIME4Rec}}}
            & \textbf{0.0607}
            & \textbf{0.0920}
            &
            & \textbf{0.0221}
            & \textbf{0.0341}
            &
            & \textbf{0.0370}
            & \textbf{0.0572}
            \\
            
            
            & \multicolumn{1}{c}{}
            & $\uparrow$10.16\%
            & $\uparrow$7.60\%
            &
            & $\uparrow$12.18\%
            & $\uparrow$14.05\%
            &
            & $\uparrow$17.46\%
            & $\uparrow$19.17\%
            \\
            
            %  下一行
            \midrule
            \multirow{3}{*}{\textbf{8-Layer}} 
            & DuoRec
            & 0.0565
            & 0.0867
            &
            & 0.0197
            & 0.0316
            &
            & 0.0299
            & 0.0460\\
            
            
            & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{SLIME4Rec}}}
            & \textbf{0.0621}
            & \textbf{0.0910}
            &
            & \textbf{0.0221}
            & \textbf{0.0342}
            &
            & \textbf{0.0365}
            & \textbf{0.0563}\\
            
            
            & \multicolumn{1}{c}{}
            & $\uparrow$9.91\%
            & $\uparrow$4.96\%
            &
            & $\uparrow$12.18\%
            & $\uparrow$8.23\%
            &
            & $\uparrow$22.07\%
            & $\uparrow$19.17\%\\
            
            %  下一行
            \midrule
            \multirow{3}{*}{\textbf{16-Layer}} 
            & DuoRec
            & 0.0517
            & 0.0790
            &
            & 0.0153
            & 0.0249
            &
            & 0.0265
            & 0.0411\\
            
            
            & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{SLIME4Rec}}}
            & \textbf{0.0585}
            & \textbf{0.0893}
            &
            & \textbf{0.0178}
            & \textbf{0.0274}
            &
            & \textbf{0.0334}
            & \textbf{0.0512}\\
            
            
            & \multicolumn{1}{c}{}
            & $\uparrow$13.15\%
            & $\uparrow$13.04\%
            &
            & $\uparrow$16.34\%
            & $\uparrow$10.04\%
            &
            & $\uparrow$26.04\%
            & $\uparrow$24.57\%\\
            
            % 底部
            \bottomrule
\end{tabular}   
    \end{adjustbox}
\end{table}


\begin{table}[t]
\renewcommand{\arraystretch}{1}
    \centering
    \label{tab:seq}
    \begin{adjustbox}{max width=\linewidth}
            \begin{tabular}{ccccccc}
            \toprule
            \multicolumn{2}{c}{\multirow{2}{*}{Method}}                               
            & \multicolumn{2}{c}{ML-1M} 
            &
            & \multicolumn{2}{c}{Yelp} \\
            \cmidrule{3-4}
            \cmidrule{6-7}
            \multicolumn{2}{c}{}
            & HR@5
            & NDCG@5
            &
            & HR@5
            & NDCG@5\\
            
            \midrule
            \midrule
            \multirow{3}{*}{\textbf{2-Layer}} 
            & DuoRec
            & 0.2038
            & 0.2946
            &
            & 0.0441
            & 0.0631\\
            
                         
            & \multirow{2}{*}{\textbf{SLIME4Rec}}
            & \textbf{0.2139}
            & \textbf{0.3026}
            &
            & \textbf{0.0516}
            & \textbf{0.0766}\\
            
                         
            &
            & $\uparrow$4.96\%
            & $\uparrow$2.72\%
            &
            & $\uparrow$0\%
            & $\uparrow$0\%\\
            
            %  下一行
            \midrule
            \multirow{3}{*}{\textbf{4-Layer}} 
            & DuoRec
            & 0.2065
            & 0.2917
            &
            & 0.0
            & 0.0\\
            
            
            & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{SLIME4Rec}}}
            & \textbf{0.2202} 
            & \textbf{0.3127}
            &
            & \textbf{0.0502} 
            & \textbf{0.0765}\\
            
            
            & \multicolumn{1}{c}{}
            & $\uparrow$6.63\%
            & $\uparrow$7.20\%
            &
            & $\uparrow$0\%
            & $\uparrow$0\%\\
            
            %  下一行
            \midrule
            \multirow{3}{*}{\textbf{8-Layer}} 
            & DuoRec
            & 0.2164
            & 0.3063
            &
            & 0.0
            & 0.0\\
            
            
            & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{SLIME4Rec}}}
            & \textbf{0.2262} 
            & \textbf{0.3132}
            &
            & \textbf{0.0493} 
            & \textbf{0.0745}\\
            
            
            & \multicolumn{1}{c}{}
            & $\uparrow$4.53\%
            & $\uparrow$2.25\%
            &
            & $\uparrow$0\%
            & $\uparrow$0\%\\
            
            %  下一行
            \midrule
            \multirow{3}{*}{\textbf{16-Layer}} 
            & DuoRec
            & 0.
            & 0.
            &
            & 0.
            & 0.\\
            
            
            & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{SLIME4Rec}}}
            & \textbf{0.2237}
            & \textbf{0.3156}
            &
            & \textbf{0.0}
            & \textbf{0.0}\\
            
            
            & \multicolumn{1}{c}{}
            & $\uparrow$\%
            & $\uparrow$\%
            &
            & $\uparrow$\%
            & $\uparrow$\%\\
            
            % 底部
            \bottomrule
\end{tabular}   
    \end{adjustbox}
\end{table}

  
